Learning Feature-Preserving Portrait Editing from Generated Pairs

Portrait editing is challenging for existing techniques due to difficulties in preserving subject features like identity. In this paper, we propose a training-based method leveraging auto-generated paired data to learn desired editing while ensuring the preservation of unchanged subject features. Specifically, we design a data generation process to create reasonably good training pairs for desired editing at low cost. Based on these pairs, we introduce a Multi-Conditioned Diffusion Model to effectively learn the editing direction and preserve subject features. During inference, our model produces accurate editing mask that can guide the inference process to further preserve detailed subject features. Experiments on costume editing and cartoon expression editing show that our method achieves state-of-the-art quality, quantitatively and qualitatively.

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Diffusion models have emerged as a powerful alternative to GAN-based methods, particularly in their ability to generate diverse imageries with superior visual quality. This advantage has spurred a wave of research exploring their application in image editing tasks. While these models have shown promise for general image editing, portrait editing presents a unique challenge. In portrait editing, maintaining identity accuracy and minimizing facial artifacts are crucial, as even minor deviations can significantly impact the perceived quality. Consequently, leveraging diffusion models for high-fidelity portrait editing remains a formidable and largely unaddressed challenge.

Most existing approaches are inference based. SDEdit~\cite{}, an influential method in this domain, produces few artifacts but struggles with structure preservation due to its global change approach. Inpainting methods~\cite{}, falter in defining appropriate masks for editing, which is particularly problematic for semantic edits like expression changes. To address this, DiffEdit~\cite{} attempts automatic mask generation, yet the resulting masks are often too noisy for high-quality portrait editing. Another approach, P2P-zero~\cite{}, embeds the mask as a regularization factor in an optimization process of the attention map but suffers from instability and inconsistency in editing results. Both DiffEdit and P2P-zero are further limited by their reliance on DDIM inversion~\cite{} or variants, struggling to balance between reconstruction fidelity and editing capability.

Recent advancements in training-based image editing have leveraged paired data to learn specific editing directions. A notable example is IP2P~\cite{}, whose effectiveness is inherently limited by the quality of its training dataset~\cite{} generated by P2P~\cite{}. In this paper, we introduce an enhanced paired data generation method that significantly improves identity preservation and structural alignment. Another approach, BBDM~\cite{}, translates latent representations across different domains. However, its network architecture falls short in effectively incorporating input information. In contrast, our research proposes a Multi-Conditioned Diffusion Model (MCDM), specifically engineered to adeptly integrate conditioning signals. This model also excels in accurately reconstructing the input image so that it can generate high quality editing masks, which can be used to guide the inference.

Our contribution is a training-based portrait editing framework to achieve better identity and structure preservation, by learning editing directions from generated paired data. Specifically, we employ Composable Diffusion~\cite{}, conditioned on both pose and identity, to create a paired dataset that is approximately aligned. The pose conditioning primarily enhances alignment, while identity conditioning augments both alignment and dataset diversity. This tailored dataset forms the foundation for training our innovative Multi-Conditioned Diffusion Model. Our model is designed to take an input image and a target prompt, effectively predicting the desired edits. It integrates conditioning signals - the image and the prompt - through multiple pathways. Our experimental results demonstrate that this method significantly enhances the consistency between the model's predictions and the given conditions. Additionally, we incorporate a reconstruction task into the training process. This enables our model to more accurately reconstruct the input image, which in turn facilitates the generation of improved masks to guide the inference process.



%In diffusion-based image editing, text prompts have unlocked new avenues for portrait customization with remarkable flexibility. Despite this, real-world scenarios often require a more focused selection of styles, such as a range of costumes for virtual try-ons or a set of expressions for cartoon stickers. Many service providers adopt predefined styles crafted by designers to meet this need and mitigate legal and quality concerns. For such applications, the emphasis shifts towards quality assurance - ensuring robust identity preservation, precise style control, and minimal unintended alterations and artifacts, taking precedence over the versatility offered by free text input.

%To this end, we trade editability for quality, by learning a specific domain of editing directions, such as costume alteration or expression modification, via synthetic data. This idea is related to data driven image-to-image translation. Previous GAN based methods~\cite{liu2022compositional} cannot easily produce results matching diffusion models' quality. A recent work BBDM~\cite{li2023bbdm} adopts a similar idea for diffusion models, but its quality is bounded by the training dataset. Despite the ability of diffusion models to produce visually striking results, generating perfectly aligned paired data remains challenging. This is particularly true for portraits, where even minor deviations in identity or slight facial artifacts are immediately noticeable and impactful.

%In this work, we introduce a novel approach to overcome the aforementioned challenge, aiming to yield high-quality identity-preserving results in portrait editing. Specifically, we employ Composable Diffusion~\cite{liu2022compositional} conditioned on pose and identity to generate an approximately but not perfectly aligned paired dataset. The pose condition is used to improve alignment while the identity condition is used to improve diversity. The paired dataset is then used for training a novel Multi-Conditioned Diffusion Model. The proposed model takes an input image and a target prompt, predicting the editing result. The conditioning signals (image and prompt) are sent into the model through multiple pathways to maintain consistency between the prediction and conditions. During inference, we propose a mask-guided strategy to ensure changes are only made to regions of interest.

Figure~\ref{fig:teaser} exemplifies the efficacy of our approach: The editing results achieves expressive styles while preserving input identity, in both real person costume and cartoon expression editing cases. The effectiveness of our method is further substantiated by quantitative analysis and user study (Sec.~\ref{sec:exp}), which collectively attest to its superiority over existing baseline methods.

To sum up, our contributions include:  (1) We design a strategically conditioned data generation technique that provides paired data with better identity and layout alignment; (2) We propose a Multi-Conditioned Diffusion Model that produces extraordinary input-output consistency and accurate editing mask for inference guidance; (3) Our approach achieves state-of-the-art portrait editing results.

% Shen, Jing, Peihao: everyone find 5 people
% Jing: solve legal issue about code release
% Tiancheng: draft introduction, abstract
% Peihao: Related work
% Bowei: 1. related work, list key works/motivation to Peihao; 2. figure 3; 3. move ablation study figure; 4. rewrite method section to match key story; 5. caption more detailed
%ddl: 13-th


==> tex/fig/costume_val_comparison.tex <==
\begin{figure*}[!h]
\begin{center}
\begin{subfigure}[b]{0.135\linewidth}
\includegraphics[width=\linewidth]{fig/experiments/costume_val/29_3/input.jpg} %
\caption{Input}
\end{subfigure}
\begin{subfigure}[b]{0.135\linewidth}
\includegraphics[width=\linewidth]{fig/experiments/costume_val/29_3/diffedit.jpg} %
\caption{DiffEdit}
\end{subfigure}
\begin{subfigure}[b]{0.135\linewidth}
\includegraphics[width=\linewidth]{fig/experiments/costume_val/29_3/sdedit 0.5.jpg} %
\caption{SDEdit 0.5}
\end{subfigure}
\begin{subfigure}[b]{0.135\linewidth}
\includegraphics[width=\linewidth]{fig/experiments/costume_val/29_3/SPADE.jpg} %
\caption{SPADE}
\end{subfigure}
\begin{subfigure}[b]{0.135\linewidth}
\includegraphics[width=\linewidth]{fig/experiments/costume_val/29_3/BBDM.jpg} %
\caption{BBDM}
\end{subfigure}
\begin{subfigure}[b]{0.135\linewidth}
\includegraphics[width=\linewidth]{fig/experiments/costume_val/29_3/ours.jpg} %
\caption{Ours}
\end{subfigure}
\begin{subfigure}[b]{0.135\linewidth}
\includegraphics[width=\linewidth]{fig/experiments/costume_val/29_3/GT.jpg} %
\caption{GT}
\end{subfigure}
\caption{Comparison of  costume editing on the validation set. The training-free baselines (b) and (c) fail to achieve the desired editing, while training-based ones (d) and (e) contain artifacts. Our method provides the best editing results.
}
\label{fig:val_baseline_comparison_costume}
\end{center}


\end{figure*}




==> tex/fig/expression_cond_ablation.tex <==
\begin{figure*}[!t]
\begin{center}
\begin{subfigure}[b]{0.16\linewidth}
\includegraphics[width=\linewidth]{fig/experiments/costume_val_ablation/input.jpg} %
\caption{Input}
\end{subfigure}
\begin{subfigure}[b]{0.16\linewidth}
\includegraphics[width=\linewidth]{fig/experiments/costume_val_ablation/ours_random.jpg} %
\caption{Ours w/o Prt}
\end{subfigure}
\begin{subfigure}[b]{0.16\linewidth}
\includegraphics[width=\linewidth]{fig/experiments/costume_val_ablation/ours_no_concat.jpg} %
\caption{Ours w/o Ipt}
\end{subfigure}
\begin{subfigure}[b]{0.16\linewidth}
\includegraphics[width=\linewidth]{fig/experiments/costume_val_ablation/ours_no_image_embeddings.jpg} %
\caption{Ours w/o Iemb}
\end{subfigure}
\begin{subfigure}[b]{0.16\linewidth}
\includegraphics[width=\linewidth]{fig/experiments/costume_val_ablation/ours.jpg} %
\caption{Ours}
\end{subfigure}
\begin{subfigure}[b]{0.16\linewidth}
\includegraphics[width=\linewidth]{fig/experiments/costume_val_ablation/GT.jpg} %
\caption{GT}
\end{subfigure}
\caption{Ablation study of  costume editing on validation set. 
}
\label{fig:costume_cond_ablation}
\end{center}
\end{figure*}




==> tex/fig/expression_val_comparison.tex <==
\begin{figure*}[!h]
\begin{center}
\begin{subfigure}[b]{0.135\linewidth}
\includegraphics[width=\linewidth]{fig/experiments/exp_val/212_val/input.jpg} %
\caption{Input}
\end{subfigure}
\begin{subfigure}[b]{0.135\linewidth}
\includegraphics[width=\linewidth]{fig/experiments/exp_val/212_val/diffedit.jpg} %
\caption{DiffEdit}
\end{subfigure}
\begin{subfigure}[b]{0.135\linewidth}
\includegraphics[width=\linewidth]{fig/experiments/exp_val/212_val/sdedit 0.5.jpg} %
\caption{SDEdit 0.5}
\end{subfigure}
\begin{subfigure}[b]{0.135\linewidth}
\includegraphics[width=\linewidth]{fig/experiments/exp_val/212_val/SPADE.jpg} %
\caption{SPADE}
\end{subfigure}
\begin{subfigure}[b]{0.135\linewidth}
\includegraphics[width=\linewidth]{fig/experiments/exp_val/212_val/BBDM.jpg} %
\caption{BBDM}
\end{subfigure}
\begin{subfigure}[b]{0.135\linewidth}
\includegraphics[width=\linewidth]{fig/experiments/exp_val/212_val/ours.jpg} %
\caption{Ours}
\end{subfigure}
\begin{subfigure}[b]{0.135\linewidth}
\includegraphics[width=\linewidth]{fig/experiments/exp_val/212_val/GT.jpg} %
\caption{GT}
\end{subfigure}
\caption{Comparison of  cartoon expression editing on the validation set. The baselines (b), (c), and (d) exhibit noticeable artifacts, and (e) fails to preserve the identity in input (a).  In contrast, our method produces high-quality editing results while preserving the identity.
}
\label{fig:val_baseline_comparison_expression}
\end{center}


\end{figure*}




==> tex/fig/main_results_exp.tex <==
\begin{figure*}[!h]
\begin{center}
\begin{subfigure}[b]{0.16\linewidth}
\includegraphics[width=\linewidth]{placeholder} %
\end{subfigure}
\begin{subfigure}[b]{0.16\linewidth}
\includegraphics[width=\linewidth]{placeholder} %
\end{subfigure}
\begin{subfigure}[b]{0.16\linewidth}
\includegraphics[width=\linewidth]{placeholder} %
\end{subfigure}
\begin{subfigure}[b]{0.16\linewidth}
\includegraphics[width=\linewidth]{placeholder} %
\end{subfigure}
\begin{subfigure}[b]{0.16\linewidth}
\includegraphics[width=\linewidth]{placeholder} %
\end{subfigure}
\begin{subfigure}[b]{0.16\linewidth}
\includegraphics[width=\linewidth]{placeholder} %
\end{subfigure}
\\
\begin{subfigure}[b]{0.16\linewidth}
\includegraphics[width=\linewidth]{placeholder} %
\end{subfigure}
\begin{subfigure}[b]{0.16\linewidth}
\includegraphics[width=\linewidth]{placeholder} %
\end{subfigure}
\begin{subfigure}[b]{0.16\linewidth}
\includegraphics[width=\linewidth]{placeholder} %
\end{subfigure}
\begin{subfigure}[b]{0.16\linewidth}
\includegraphics[width=\linewidth]{placeholder} %
\end{subfigure}
\begin{subfigure}[b]{0.16\linewidth}
\includegraphics[width=\linewidth]{placeholder} %
\end{subfigure}
\begin{subfigure}[b]{0.16\linewidth}
\includegraphics[width=\linewidth]{placeholder} %
\end{subfigure}
\\
\begin{subfigure}[b]{0.16\linewidth}
\includegraphics[width=\linewidth]{placeholder} %
\caption{Real Photo}
\end{subfigure}
\begin{subfigure}[b]{0.16\linewidth}
\includegraphics[width=\linewidth]{placeholder} %
\caption{Cartoonized Input}
\end{subfigure}
\begin{subfigure}[b]{0.16\linewidth}
\includegraphics[width=\linewidth]{placeholder} %
\caption{angry}
\end{subfigure}
\begin{subfigure}[b]{0.16\linewidth}
\includegraphics[width=\linewidth]{placeholder} %
\caption{laughing}
\end{subfigure}
\begin{subfigure}[b]{0.16\linewidth}
\includegraphics[width=\linewidth]{placeholder} %
\caption{crying}
\end{subfigure}
\begin{subfigure}[b]{0.16\linewidth}
\includegraphics[width=\linewidth]{placeholder} %
\caption{shocked}
\end{subfigure}
\caption{Our costume editing  results on real image. 
}
\label{fig:baseline_comparison}
\end{center}

\end{figure*}






==> tex/table/experiments/metrics_bk.tex <==
\begin{table}[]
\begin{tabular}{|l|l|l|l|l|}
\hline
\multicolumn{5}{|c|}{Costume Editing Dataset} \\ \hline
             & RMSE           & SSIM           & LPIPS          & FID \\ \hline
p2p          & 0.265          & 0.823          & 0.636          &     \\ 
pix2pix-zero & 0.328          & 0.754          & 0.751          &     \\ 
diffedit     & 0.305          & 0.781          & 0.667          &     \\ \hline
sdedit 0.8   & 0.324          & 0.746         & 0.702         &     \\ \hline
sdedit 0.5   & 0.305          & 0.778         & 0.657          &     \\ \hline
SPADE        & 0.290        & 0.820          & 0.599          &     \\ \hline
BBDM         & 0.284          & 0.830          & 0.614          &     \\ \hline
Ours         & \textbf{0.277} & \textbf{0.864} & \textbf{0.577} &     \\ \hline
\multicolumn{5}{|c|}{Expression Editing Dataset} \\ \hline
             & RMSE           & SSIM           & LPIPS          & FID \\ \hline
p2p          & 0.159          & 0.923          & 0.413          &     \\ \hline
pix2pix-zero & 0.219          & 0.896          & 0.635          &     \\ \hline
diffedit     & 0.164          & 0.928          & 0.407          &     \\ \hline
sdedit 0.8   & 0.184         & 0.913          & 0.466          &     \\ \hline
sdedit 0.5   & 0.162         & 0.928          & 0.426          &     \\ \hline
SPADE        & 0.156          & 0.927          & 0.412          &     \\ \hline
BBDM         & 0.152         & 0.935          & 0.400          &     \\ 
\hline
Ours         & \textbf{0.277} & \textbf{0.946} & \textbf{0.394} &     \\ \hline
\end{tabular}
\caption{Quantitative results on costume dataset}
\end{table}
